Learning Software Constraints via Installation Attempts

Modern software systems are expected to be secure and contain all the latest features, even when new versions of software are released multiple times an hour. Each system may include many interacting packages. The problem of installing multiple dependent packages has been extensively studied in the past, yielding some promising solutions that work well in practice. However, these assume that the developers declare all the dependencies and conflicts between the packages. Oftentimes, the entire repository structure may not be known upfront, for example when packages are developed by different vendors. In this paper, we present algorithms for learning dependencies, conflicts and defective packages from installation attempts. Our algorithms use combinatorial data structures to generate queries that test installations and discover the entire dependency structure. A query that the algorithms make corresponds to trying to install a subset of packages and getting a Boolean feedback on whether all constraints were satisfied in this subset. Our goal is to minimize the query complexity of the algorithms. We prove lower and upper bounds on the number of queries that these algorithms require to make for different settings of the problem.

==> adaptiveConflictsWithKnownDependencies.tex <==
\section{Proof of Theorem~\ref{thm:adaptiveConflictsWithKnownDependencies}}\label{app:adaptiveConflictsWithKnownDependencies}
\begin{theorem*}
	Assume that the repository contains at most $d$ defects and $c$ weak conflicts.
	There exists an \textbf{adaptive} algorithm that solves \learnAll{} using $\parameterizedCFFSize{d+c}{1}+\parameterizedCFFSize{c}{2}$ queries.
\end{theorem*}
\begin{proof}
	The idea behind our algorithm is first to identify the defects, remove them from the repository and then follow the non-adaptive procedure when no defects exist.
	Recall that in the proof of
	Lemma~\ref{lem:defectIdentificationWithConflictsKnownDependencies}, the size of
	$S_2$ was just one (only the package for which we wish to assert
	defectiveness).
	Hence, Lemma~\ref{lem:defectIdentificationWithConflictsKnownDependencies} also
	holds for \parameterizedCFFSize{d+c}{1}. Therefore, by taking a
	\parameterizedCFF{d+c}{1} and propagating the known dependencies, we can find all defects.
	The adaptivity then allows us to compute the subsequent \parameterizedCFF{c}{2}
	only on the non-defective packages and learn all conflicts.
\end{proof}

==> adaptiveMaxInstallation.tex <==
\section{Proof of Theorem~\ref{thm:adaptiveMaxInstallation}}\label{app:adaptiveMaxInstallation}
\begin{theorem*}
	Assume that the repository contains at most $d$ defects and $u$ unknown dependencies.
	Any \textbf{adaptive} algorithm for \maxProblem{} must make $\Omega\parentheses{{u+d\choose d}+d\logp{n/d}}$ queries.
\end{theorem*}
\begin{proof}
	First, note that a $d\logp{n/d}$ lower bound immediately follows from the group testing lower bound (as the case of $K=U=\emptyset$ degenerates to group testing).
	Fix an arbitrary package subset $P'\subseteq P$ of size $|P'|=u+d$. Consider an algorithm that makes at most ${u+d\choose d}-2$ queries.
	Clearly, there are ${u+d\choose d}$ subsets of size $u$ of $P'$.
	Thus, there exists two disjoint-subsets pairs $A_1,A_2\subseteq P'$ and $B_1,B_2\subseteq P'$ such that $|A_1|=|B_1|=d$ and $|A_2|=|B_2|=u$ (also, $A_1\cap A_2=B_1\cap B_2=\emptyset$) and that no tested installation contains $A_2$ but none of $A_1$ and no test includes $B_2$ but none of $B_1$.
	Consider the following scenarios:
	\begin{enumerate}[I]
		\item The set of defects is $D=A_1$ and all of the packages in $A_2$ depend on each other (i.e., there is a cycle that contains all of $A_2$ in $(P, U)$).
		\item The set of defects is $D=B_1$ and all of the packages in $B_2$ depend on
		each other (there is a cycle that contains all of $B_2$ in $(P, U)$).
	\end{enumerate} 
	Notice that in case I, any installation that contains $A_2$ but none of the packages in $A_1$ passes and similarly for case II and $B_1, B_2$. As no such installations were tested by the algorithm, every test that contains at least one package of $P'$ fails, regardless of the actual scenario. Thus, the algorithm cannot determine whether $A_2$ or $B_2$ belongs to the maximal installation and thus fails to solve the~problem.
\end{proof}

==> contributionTable.tex <==
\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\begin{table*}
	\centering
	\footnotesize
	%	\tabcolsep=0.11cm
	\begin{tabular}{|l|c|c|c|}
		\hline
		Scenario& Problem Variant& Lower bound &  Upper bound		 \\ \hline\hline
		\multirow{3}{*}{\specialcell[l]{\noindent Adaptive with at most $r$ root\\ defects and no unknown\\ dependencies or conflicts}} & \multirow{3}{*}{\learnAll{}}& \multirow{2}{*}{$\ceil{\log_2\parentheses{\sum_{i=0}^{r}{n\choose i}}}=O(r\logp{\frac{n}{r}})$} & \multirow{2}{*}{$r-1 + \ceil{\log_2\parentheses{\sum_{i=0}^{r}{n\choose i}}}$} \\&&&\\
		&& Theorem~\ref{thm:GTLB} & Theorem~\ref{thm:knownDependenciesUpperBound}\\\hline
		\multirow{2}{*}{\specialcell[l]{\noindent Adaptive, most $1$ unknown\\ dependency and $1$ root defect}} &{\sc Maximal} & $n$ & \\
		&{\sc Sub-repository}& Theorem~\ref{thm:oneRootOneUnknownDep} & \\\hline
		\multirow{3}{*}{\specialcell[l]{\noindent Non-adaptive with at\\ most $d$ defects and $u$ unknown\\ dependencies, no conflicts}} &{\sc Maximal}& \multirow{2}{*}{$\parameterizedCFFSize{d-1}{u+1}=\Omega^*(\log n)$} & \multirow{2}{*}{$\parameterizedCFFSize{d}{u+1}$} \\&{\sc Sub-repository}&&\\&
		& Theorem~\ref{thm:unknownDependenciesLB} & Theorem~\ref{thm:unknownDependenciesUB}\\\hline		
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with $1$ \\unknown dependency  and\\ no conflicts or defects}} &\multirow{3}{*}{\learnAll{}} & \multirow{2}{*}{$n-1$} & \\&&&\\
		&& Theorem~\ref{thm:learningADependency} & \\\hline		
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with $u$ \\unknown weak dependencies,\\ $c$ weak conflicts, and $d$  defects}} &{\sc Maximal} & \multirow{2}{*}{$\parameterizedCFFSize{d+\ceil{c/2}-1}{u+1}$} & \\&{\sc Sub-repository}&&\\
		&& Theorem~\ref{thm:maxLowerBoundWithConflicts} & \\\hline		
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with $u$ \\unknown weak dependencies,\\ $c$ weak conflicts, and $d$  defects}} &\multirow{3}{*}{\learnAll{}} & \multirow{2}{*}{$\parameterizedCFFSize{d+c-1}{u+1}$} & \multirow{2}{*}{$\parameterizedCFFSize{d+c+u-1}{u+1}$}\\&&&\\
		&& Theorem~\ref{thm:learnAllLBWithConflictsLB} &  Theorem~\ref{thm:learnAllLBWithConflictsUB} \\\hline				
	\end{tabular}\smallskip
	\normalsize
	\caption{Summary of our results learning undocumented constraints. Here, $\CFFSizeLetter_{\CFFParams}$ is the size of a \CFF{} as described in Section~\ref{sec:CFFs}. Recall that every algorithm for \learnAll{} also solves \maxProblem{} and every lower bound for \maxProblem{} holds for \learnAll{}.}
	\label{tbl:summary}
\end{table*} 

==> contributionTable1_tosem_bck.tex <==
\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\begin{table*} 
	\centering
	\scriptsize
%\small
	%	\tabcolsep=0.11cm
	\begin{tabular}{|l|c|l|l|c|}
		\hline
		\textbf{Scenario}& \textbf{Adaptive}& \textbf{Problem Variant}& \textbf{Query Complexity Bounds} &  \textbf{Theorem} \#		 \\
		\hline\hline \multirow{3}{*}{\specialcell[l]{\noindent At most
		$r$ root\\ defects and no unknown\\ dependencies or conflicts}} & \multirow{3}{*}{\cmark} &
		\multirow{3}{*}{\learnAll{}}&
		Lower: $\ceil{\log_2\parentheses{\sum_{i=0}^{r}{n\choose
		i}}}=\Omega(r\logp{\frac{n}{r}})$ & \ref{thm:GTLB} \\&&&&\\
		&&& Upper: $r-1 + \ceil{\log_2\parentheses{\sum_{i=0}^{r}{n\choose
		i}}}$  &
		\ref{thm:knownDependenciesUpperBound}\\\hline
		\multirow{2}{*}{\specialcell[l]{\noindent At most $1$
		unknown
		dependency\\ and $1$ root defect}}& \multirow{2}{*}{\cmark} &{\sc Maximal} & \multirow{2}{*}{Lower:
		$n=\Omega(n)$} & \multirow{2}{*}{\ref{thm:oneRootOneUnknownDep}}\\
		&&{\sc Sub-repository}&  &  \\\hline
		\multirow{5}{*}{\specialcell[l]{\noindent At most $d$
		defects and $u$\\ unknown dependencies,\\ no conflicts}}& \multirow{3}{*}{\xmark} &&
		Lower: $\parameterizedCFFSize{d-1}{u+1}=\Omega^*(\log n)$ &
		\ref{thm:unknownDependenciesLB}   \\&&{\sc Maximal}&&\\& &{\sc Sub-repository}&
		Upper: $\parameterizedCFFSize{d}{u+1}=O^*(\log n)$ &
		\ref{thm:unknownDependenciesUB}\\\hhline{~-~--}
		 & \multirow{2}{*}{\cmark}&&
		\multirow{2}{*}{Lower: $\Omega\parentheses{{u+d\choose d}+d\logp{n\over d}}=\Omega^*(\log n)$} &
		\multirow{2}{*}{\ref{thm:adaptiveMaxInstallation}}\\&&&&\\\hline	
%		{thm:learningAStrongConflict}
		\multirow{2}{*}{\specialcell[l]{\noindent At most $1$ conflict and no\\ defects or unknown dependencies}} & \multirow{2}{*}{\xmark}&\multirow{2}{*}{\learnAll{}} &
		\multirow{2}{*}{Lower: $n-1=\Omega(n)$} &
		\multirow{2}{*}{\ref{thm:learningAStrongConflict}}\\
		&&&& \\\hline	
		\multirow{5}{*}{\specialcell[l]{\noindent At most
				$c$ weak\\ conflicts, $d$ defects and\\ no unknown dependencies}}& \multirow{3}{*}{\xmark} &
		\multirow{5}{*}{\learnAll{}}&
		Lower: $\parameterizedCFFSize{d+c-1}{2}=\Omega^*(\log n)$ & \ref{thm:learnAllLBWithConflictsKnownDependenciesLB} \\&&&&\\
		&&& Upper: $\parameterizedCFFSize{d+c}{2}=O^*(\log n)$  &
		\ref{thm:learnAllLBWithConflictsUBKnownDependencies}\\\hhline{~-~--}	
		& \multirow{2}{*}{\cmark}&&
		\multirow{2}{*}{Upper: $\parameterizedCFFSize{d+c}{1}+\parameterizedCFFSize{c}{2}=O^*(\log n)$} &
		\multirow{2}{*}{\ref{thm:adaptiveConflictsWithKnownDependencies}}\\
		&&&& \\\hline				
		\multirow{2}{*}{\specialcell[l]{\noindent At most $1$ unknown
		dependency\\ and no conflicts or defects}} &
		\multirow{2}{*}{\xmark}&\multirow{2}{*}{\learnAll{}} & \multirow{2}{*}{Lower:
		$n-1=\Omega(n)$} & \multirow{2}{*}{\ref{thm:learningADependency}}\\
	&&&& \\\hline				
		\multirow{7}{*}{\specialcell[l]{\noindent At most $u$ unknown\\
				dependencies, $c$ conflicts,\\ and $d$  defects.}} & \multirow{7}{*}{\xmark}&{\sc Maximal} &
		\multirow{2}{*}{Lower:
		$\parameterizedCFFSize{d+\ceil{c/2}-1}{u+1}=\Omega^*(\log n)$} & \multirow{2}{*}{\ref{thm:maxLowerBoundWithConflicts}} \\&&{\sc
		Sub-repository}&&\\\hhline{~~---}		
		&
		&\multirow{5}{*}{\learnAll{}} & Lower:
		$\parameterizedCFFSize{d+c-1}{u+2}=\Omega^*(\log n)$ &\ref{thm:learnAllLBWithConflictsV2} \\&&&&\\
		&&&
		Upper: 
		$\!\begin{aligned} % http://tex.stackexchange.com/q/98482/16595 
		&\sum_{i=0}^{u}\parameterizedCFFSize{d+c+(u-i)+1}{i+2} \\    % http://tex.stackexchange.com/q/78788/16595
		&< \parameterizedCFFSize{d+c+u+1}{u+2}=O^*(\log n) \end{aligned}$
		& 
		\ref{thm:learnAllLBWithConflictsUB} \\\hline \end{tabular}\smallskip
	\normalsize
	\caption{Summary of our results learning undocumented constraints. Here, $\CFFSizeLetter_{\CFFParams}$ is the size of a \CFF{} as described in Section~\ref{sec:CFFs}. Recall that every algorithm for \learnAll{} also solves \maxProblem{} and every lower bound for \maxProblem{} holds for \learnAll{}.}
	\label{tbl:summary}
%	\vspace{-.5cm}
\end{table*} 

==> contributionTable2.tex <==
\begin{table*}
	\centering
	\footnotesize
	%	\tabcolsep=0.11cm
	\begin{tabular}{|l|l|l|}
		\hline
		Scenario& Problem Variant& Bounds for Query Complexity		 \\ \hline\hline
		\multirow{3}{*}{\specialcell[l]{\noindent Adaptive with at most $r$ root\\
		defects and no unknown\\ dependencies or conflicts}} &
		\multirow{3}{*}{\learnAll{}}&
		Lower: $\ceil{\log_2\parentheses{\sum_{i=0}^{r}{n\choose
		i}}}=O(r\logp{\frac{n}{r}})$ (Theorem~\ref{thm:GTLB}) \\&&\\
		&&  Upper: $r-1 + \ceil{\log_2\parentheses{\sum_{i=0}^{r}{n\choose
		i}}}$  (Theorem~\ref{thm:knownDependenciesUpperBound})\\\hline
		\multirow{2}{*}{\specialcell[l]{\noindent Adaptive, most $1$ unknown\\
		dependency and $1$ root defect}} &{\sc Maximal} & \multirow{2}{*}{Lower: $n$
		(Theorem~\ref{thm:oneRootOneUnknownDep})}  \\
		&{\sc Sub-repository}&  \\\hline
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with at\\ most $d$
		defects and $u$ unknown\\ dependencies, no conflicts}} &{\sc Maximal}& \multirow{2}{*}{$\parameterizedCFFSize{d-1}{u+1}=\Omega^*(\log n)$}  \multirow{2}{*}{$\parameterizedCFFSize{d}{u+1}$} \\&{\sc Sub-repository}&\\& & Theorem~\ref{thm:unknownDependenciesLB}  Theorem~\ref{thm:unknownDependenciesUB}\\\hline		
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with $1$ \\unknown dependency  and\\ no conflicts or defects}} &\multirow{3}{*}{\learnAll{}} & \multirow{2}{*}{$n-1$}  \\&&\\
		&& Theorem~\ref{thm:learningADependency}  \\\hline		
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with $u$ \\unknown weak dependencies,\\ $c$ weak conflicts, and $d$  defects}} &{\sc Maximal} & \multirow{2}{*}{$\parameterizedCFFSize{d+\ceil{c/2}-1}{u+1}$}  \\&{\sc Sub-repository}&\\
		&& Theorem~\ref{thm:maxLowerBoundWithConflicts}  \\\hline		
		\multirow{3}{*}{\specialcell[l]{\noindent Non-Adaptive with $u$ \\unknown weak dependencies,\\ $c$ weak conflicts, and $d$  defects}} &\multirow{3}{*}{\learnAll{}} & \multirow{2}{*}{$\parameterizedCFFSize{d+c-1}{u+1}$}  \multirow{2}{*}{$\parameterizedCFFSize{d+c+u-1}{u+1}$}\\&&\\
		&& Theorem~\ref{thm:learnAllLBWithConflictsLB}   Theorem~\ref{thm:learnAllLBWithConflictsUB} \\\hline				
	\end{tabular}\smallskip
	\normalsize
	\caption{Summary of our results learning undocumented constraints. Here, $\CFFSizeLetter_{\CFFParams}$ is the size of a \CFF{} as described in Section~\ref{sec:CFFs}. Recall that every algorithm for \learnAll{} also solves \maxProblem{} and every lower bound for \maxProblem{} holds for \learnAll{}.}
	\label{tbl:summary}
\end{table*} 

==> defectIdentificationWithConflicts.tex <==
\section{Proof of Lemma~\ref{lem:defectIdentificationWithConflicts}}\label{app:defectIdentificationWithConflicts}
\begin{lemma*}
	A package $p\in P$ is defective if and only if $S(p)=\emptyset$.
\end{lemma*}
\begin{proof}
	The difference between the model here and that of Lemma~\ref{lem:defectIdentificationWithConflictsKnownDependencies} is that we now allow unknown dependencies and assume that $K=\emptyset$.
	As before, a defective package $p$ yields $S(p)=\emptyset$; we show that if $p\notin D$ then we have a successful test that includes $p$ to witness that.
	Intuitively, we satisfy each conflict by excluding (having in $S_1$) one of its 
	packages along with all those that depend on it. Unlike before, we split our unknown dependency resolution to cases. We wish to have all packages that $p$ 
	weakly depends on active (i.e., in $S_2$). All other packages that have an
	unknown dependency are excluded (placed in $S_1$), and so are all the packages
	that depend on them.
	The setting is illustrated in Figure~\ref{fig:defectIdentificationIllustration}.
	
	%Unlike Lemma~\ref{lem:defectIdentificationWithConflictsKnownDependencies}, we now need to add to $S_2$ all of the prerequisites of $p$. That is, we set $S_2\triangleq\set{p'\mid \mbox{$p$ has a weak dependency on $p'$}}$. Notice that we have $S_2\le u+1 < u+2$ as needed.
	%The claim is similar to Lemma~\ref{lem:defectiveness} except that now we may have conflicts. Once again, if $p$ is defective then clearly $S(p)=\emptyset$, and our goal to show the converse.
	%Intuitively, we can satisfy the conflict constraints by excluding all packages that cannot be successfully installed jointly with $p$ and by excluding one package of each weak conflict that does not relate to $p$.
	%
	%
	Next, notice that if $p$ weakly depends on two packages $p',p''$ that conflict, then $p$ cannot be successfully installed and is thus a defect. Therefore, we hereafter assume that no two packages that $p$ weakly depends on conflict.
	%Formally, consider a partition of the conflicts into those that affect $p$ and those that do not, i.e., $C=C_1\cup C_2$, $C_1\triangleq\set{\set{q,p'}\mid q,p'\in P, p\mbox{ has a weak dependency on } p'}, C_2\triangleq C\setminus C_1$. 
	
	%The rest of the proof contains a formal definition of disjoint sets $S_1, S_2$ such that the test that corresponds to the pair includes $p$ and passes.
	Following are formal definitions of sets $S_1, S_2$ such that the test that
	contains $S_2$ and avoids $S_1$ succeeds, thus serving as a witness to the
	non-defectiveness of $p$.
	We define $S_2$ as $p$ and all of the the packages it depends on:
	$S_2\triangleq\set{p}\cup\set{p'\mid\mbox{$p$ has an \textbf{unknown}
	weak dependency on $p'$}}$.
	Once again, we consider some order $\succ$ on $P$ for resolving the conflicts. 
	We define three package sets as follows:
	%$S_1 = D\cup S_1'\cup S_1''\cup S_1'''$, where 
	\begin{itemize}
		\item $X_1\triangleq \set{q\mid \mbox{($p$ does not weakly depend on $q$)}\wedge(\exists p'\in P: (p',q)\in U)}$.
		\item $X_2\triangleq \set{q\mid \exists p':(\set{q,p'}\in C) \wedge(\mbox{$p$ weekly depends on $p'$})}$.
		\item $X_3\triangleq \set{q\mid \exists p':(\set{q,p'}\in C) \wedge\mbox{($p$ does not weekly depends on $q$)}\wedge(q\succ p')}$.
	\end{itemize} 
	
	Intuitively, $X_1$ is the set of packages that have an unknown dependency and are not a prerequisite to $p$. $X_2$ contains all packages that conflict with a prerequisite of $p$. $X_3$'s packages are those that have no relation to $p$ and has an unknown conflict with another package with a lower index according to $\succ$.
	If we make sure that we have a test that installs all of $p$'s prerequisites and excludes all packages in $X_1\cup X_2\cup X_3$, it will pass unless $p$ is defective. 
	Thus, we define $S_1\triangleq D\cup X_1\cup X_2\cup X_3$.
	%However, due to the propagation of the known dependencies, it is not enough to include \textit{just} $E$ in $S_1$. That is, if a package $q$ in $E$ is a member of $S_1$, but a package that depends on it has $1$ in the corresponding vector $v$, the propagation-result $c(v)$ will include $q$ as well. We circumvent this issue by adding to $S_1$ \textit{all} packages that weekly depends on $E$, i.e., we set $S_1\triangleq D\cup \set{q\mid \exists q'\in E: \mbox{$q$ weakly depends on $q'$}}$. Since every package in $S_1$ has an unknown weak conflict or dependency we have that $|S_1|\le d+c+u$. Figure~\ref{fig:defectIdentificationIllustration} illustrates the sets $S_1,S_2$ that allow the corresponding test $c(v)$ to pass if $p$ is not defective.
		%For resolving the constraints that affect $p$ we need a test that excludes
	%$S_{1,1}\triangleq\set{q\mid \exists p':(q,p')\in C\wedge p\mbox{ has a weak dependency on } p'}$. Next, consider some canonical ordering $(\succ)$ over the packages and define $S_{1,2}\triangleq\set{q\mid \exists p':(q,p')\in C\wedge (q\succ p')\wedge p\mbox{ has a no week dependencies on } p' \mbox {or q}}$. That is, we arbitrarily choose the package we wish to exclude $q$ with respect to the order $\succ$. The two sets, together with all defects, form the exclusion set required for a test in $T(p)$ to pass and thus we define $S_1\triangleq S_{1,1}\cup S_{1,2}\cup D$. Observe that the size of $S_1$ is at most $d+c$ and not $d+c+u$; while this allows use to identify the defects using fewer queries, the additional $u$ exclusions will come handy for learning the dependencies and conflicts. Next, we need to define the inclusion set $S_2$. Once again, this is done similarly to the previous section and we add to it all non-defective packages that are a prerequisite to another package; formally, $S_2\triangleq\set{p}\cup\set{p'\in (P\setminus D)\mid \exists p''\in P, (p',p'')\in U}$. The size of $S_2$ is at most the one plus the number of dependencies which may be smaller than the number of weak dependencies. Nevertheless, the weak dependencies prove vital for identifying the missing dependencies and conflicts. 
	\begin{figure}[]
		\centering
		\includegraphics[width =
		0.75\columnwidth]{figs/defectIdentificationIllustration.png}
		
		\caption{An example of a $S_1,S_2$ whose corresponding test contains 
		$p$ and passes. $S_2$ contains $p$ and all of its prerequisites. $S_1$
		contains all packages that weakly conflict with $p$, all packages $q$ that are not a 
		prerequisite to $p$ and have an unknown dependency, and a package from each
		conflict, chosen according to $\succ$.
		}
		\label{fig:defectIdentificationIllustration}
	\end{figure}
	Observe that every package in $S_1$ can be uniquely associated with a defect, conflict or dependency.
	Thus, we have $|S_1|\le d+c+u<d+c+u+1$ and $S_2\le u+1<u+2$ and hence there exists a vector $v\in\CFFLetter$ (and subsequently, a test) such that $S_1\cap v=\emptyset$ and $S_2\subseteq v$. By the construction of $S_1$ and $S_2$ we are guaranteed that the test includes $p$ and satisfies all conflict and dependency constrains.
\end{proof}


==> defectIdentificationWithConflictsKnownDependencies.tex <==
\section{Proof of Lemma~\ref{lem:defectIdentificationWithConflictsKnownDependencies}}\label{app:defectIdentificationWithConflictsKnownDependencies}
\begin{lemma*}
	A package $p\in P$ is defective if and only if $S(p)=\emptyset$.
\end{lemma*}
\begin{proof}
	The claim is similar to Lemma~\ref{lem:defectiveness} except that now we may
	have conflicts, and all the dependencies are known. Once again, if $p$ is
	defective, then clearly $S(p)=\emptyset$, and our goal is to show the converse.
	Given a non-defective $p$, we construct sets $S_1, S_2$ of the required sizes
	such that a test containing all of $S_2$ and none of $S_1$ succeeds, thus
	showing that $S(p) \neq \emptyset$.
	%Intuitively, we can satisfy the conflict constraints by excluding all packages that cannot be successfully installed jointly with $p$ and by excluding one package of each weak conflict that does not relate to $p$.
	Intuitively, we satisfy each conflict by excluding (having in $S_1$) one of its packages along with all those that depend on it. 
	As for $S_2$, all we need is to include $p$ as the dependency propagation will ensure that all its prerequisites are installed as well.
	%Unlike before, we split our unknown dependency resolution to cases. We wish to have all packages that $p$ weakly depend on active (i.e., in $S_2$). All other packages that have an unknown dependency are \emph{excluded} (placed in $S_1$), and so are all the packages that depend on them.
	The setting is illustrated in Figure~\ref{fig:defectIdentificationIllustrationKnownDependencies}.
	
	Next, notice that if $p$ weakly conflicts with a prerequisite of its, 
	then $p$ cannot be successfully installed and is thus a defect. Hence, we
	hereafter assume that $p$ does not conflict with any of its prerequisites.
	%Formally, consider a partition of the conflicts into those that affect $p$ and those that do not, i.e., $C=C_1\cup C_2$, $C_1\triangleq\set{\set{q,p'}\mid q,p'\in P, p\mbox{ has a weak dependency on } p'}, C_2\triangleq C\setminus C_1$. 
	We now formally define a pair of disjoint 
	sets $S_1, S_2$ such that the corresponding test contains $p$ and passes.
	Here, $S_2 = \set{p}$.
	%We define $S_2=\set{p}$; that is, it contains $p$ and the set of packages needed so that taking all their \textit{known} prerequisites satisfies all $p$'s prerequisites.
	Next, we consider an arbitrary order $\succ$ on $P$ that will allow us to resolve the conflict constraints. 
	We define two package sets as follows:
	%$S_1 = D\cup S_1'\cup S_1''\cup S_1'''$, where 
	\begin{itemize}
		\item $X_1\triangleq \set{q\mid \exists p':\set{q,p'}\in C \wedge\mbox{$p$ weekly depends on $p'$}}$.
		\item $X_2\triangleq \set{q\mid \exists p':(\set{q,p'}\in C) \wedge\mbox{($p$ does not weekly depend on $q$)}\wedge(q\succ p')}$.
	\end{itemize} 
	
	
	Intuitively, $X_1$ contains all packages that conflict with a prerequisite of $p$; $X_2$'s packages are those that have no relation to $p$ and have an unknown conflict with another package with a lower index (according to $\succ$).
	If we make sure that we have a test that installs all of $p$'s prerequisites
	and excludes all packages in $E\triangleq X_1\cup X_2$, it will pass if $p$ is not defective. 
	However, due to the propagation of the known dependencies, it is not enough to 
	include \textit{just} $D\cup E$ in $S_1$. That is, if a package $q\in E$ is a member 
	of $S_1$, but a package that depends on it has `$1$` in the corresponding
	vector $v$ in the CFF, the propagation-result $c(v)$ will include $q$ as well.
	We circumvent this issue by adding to $S_1$ \textit{all} packages that weekly depend on $E$, i.e., we set $S_1\triangleq D\cup \set{q\mid \exists q'\in E: \mbox{$q$ weakly depends on $q'$}}$. Since every package in $S_1$ has an unknown weak conflict or defect we have that $|S_1|\le d+c$. Figure~\ref{fig:defectIdentificationIllustrationKnownDependencies} illustrates the sets $S_1,S_2$ that allow the corresponding test $c(v)$ to pass if $p$ is not defective.
	\begin{figure}[h]
		\centering
		\includegraphics[width = 0.6\columnwidth]{figs/defectIdentificationIllustrationKnownDependencies.png}
		
		\caption{An example of a $S_1,S_2$ whose corresponding test 
		contains $p$ and passes. 
		$S_2$ contains $p$, while $S_1$ contains all packages that weakly 
		conflict with $p$ and a package from each conflict, 
		along with all those that weakly depend on it. The latter are selected based
		on the order $\succ$, such that $a_1$ is selected to be in $S_1$ first, along
		with its prerequisite $a_5$, followed by $a_2$ and $a_3$.
		}
		\label{fig:defectIdentificationIllustrationKnownDependencies}
	\end{figure}
	Since we have $|S_1|\le d+c$ and $|S_2|=1<2$ there exists a vector
	$v\in\CFFLetter$, such that $S_1\cap v=\emptyset$ and $S_2\subseteq v$. By the
	construction of $S_1$ and $S_2$ we are guaranteed that the test includes $p$ and satisfies all conflict and dependency constrains.
\end{proof}


==> evaluation.tex <==
\newcommand{\FRHHH}{10-RHHH}
\section{Evaluation}
\label{sec:eval}


==> graphs.tex <==
%\begin{figure*}[t]
%	\captionsetup{justification=centering}
%	\begin{tabular}{ccc}
%	\subfloat[\label{FPR:SJ:Byte}SanJose14 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]	{FPRGraphs/SJ14_bytes.png}} &	
%	\subfloat[SanJose14\label{FPR:SJ:bit} - 1D Bits]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/SJ14_bits.png}} &
%	\subfloat[SanJose14\label{FPR:SJ:2Dbyte} - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/SJ14_2Dbytes.png}}
%	\tabularnewline
%	\multicolumn{3}{c}{\subfloat{\includegraphics[width = 17cm]
%			{BarsLegend.png}}}		
%	\tabularnewline
%	\addtocounter{subfigure}{-1}
%	\subfloat[\label{FPR:CHI:byte}\label{FPR:`}Chicago16 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/CH16_bytes.png}} &	
%	\subfloat[\label{FPR:CHI:bit}Chicago16 - 1D Bits]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/CH16_bits.png}} &
%	\subfloat[\label{FPR:CHI:2Dbyte}Chicago16 - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/CH16_2Dbytes.png}}
%	
%\end{tabular}
%	\caption{	\label{fig:acc} Accuracy error ratio -- HHH candidates whose frequency estimation error is larger than $N\epsilon$ ($\epsilon =0.001$).}		
%	%\end{figure*}	
%	%\thisfloatsetup{subfloatrowsep=qquad}
%	%\begin{figure*}[h]	
%	\captionsetup{justification=centering}
%	\begin{tabular}{cccc}
%		\multicolumn{4}{c}{\subfloat{\includegraphics[width = 7cm, height=0.6cm]
%				{ACCCOVLegend.png}}}
%		\tabularnewline
%		\addtocounter{subfigure}{-1}
%		\subfloat[Chicago15\label{COV:CH15:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{CH15_2Dbytes_cov.png}}  &
%		\subfloat[Chicago16\label{COV:CH16:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{CH16_2Dbytes_cov.png}}  &
%		\subfloat[SanJose13\label{COV:SJ13:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{SJ13_2Dbytes_cov.png}}  &
%		\subfloat[SanJose14\label{COV:SJ14:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{SJ14_2Dbytes_cov.png}}   	
%		
%	\end{tabular}
%	\caption{\label{fig:cov} The percentage of Coverage errors -- elements $q$ such that  $q\notin P$ and $C_{q\mid P}\ge N\theta$ (false negatives).
%		%		The X axis represents the number of packets.
%	}
%\end{figure*}
%\endinput
\begin{figure*}[t]
	\begin{tabular}{ccc}
		\subfloat[\label{FPR:SJ:Byte}SanJose14 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]	{FPRGraphs/SJ14_bytes.png}} &	
		\subfloat[SanJose14\label{FPR:SJ:bit} - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/SJ14_bits.png}} &
		\subfloat[SanJose14\label{FPR:SJ:2Dbyte} - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/SJ14_2Dbytes.png}}
		\tabularnewline
		\multicolumn{3}{c}{\subfloat{\includegraphics[width = 17cm]
				{BarsLegend.png}}}		
		\tabularnewline
		\addtocounter{subfigure}{-1}
		\subfloat[\label{FPR:CHI:byte}\label{FPR:`}Chicago16 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/CH16_bytes.png}} &	
		\subfloat[\label{FPR:CHI:bit}Chicago16 - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/CH16_bits.png}} &
		\subfloat[\label{FPR:CHI:2Dbyte}Chicago16 - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/CH16_2Dbytes.png}}
		
	\end{tabular}
	\caption{	\label{FPR:fig:FPR} False Positive Rate for different stream lengths.}
\end{figure*}



\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[\label{SJ:Byte}SanJose14 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/SJ14_bytes.png}} &	
		\subfloat[SanJose14\label{SJ:bit} - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/SJ14_bits.png}} &
		\subfloat[SanJose14\label{SJ:2Dbyte} - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/SJ14_2Dbytes.png}}
		\tabularnewline
		\multicolumn{3}{c}{\subfloat{\includegraphics[width = 17cm]
				{BarsLegend.png}}}		
		\tabularnewline
		\addtocounter{subfigure}{-1}
		\subfloat[\label{CHI:byte}\label{`}Chicago16 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/CH16_bytes.png}} &	
		\subfloat[\label{CHI:bit}Chicago16 - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/CH16_bits.png}} &
		\subfloat[\label{CHI:2Dbyte}Chicago16 - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/CH16_2Dbytes.png}}
		
	\end{tabular}
	\caption{	\label{fig:speed} Update speed comparison for different hierarchical structures and workloads}
\end{figure*}


==> learnAllLBWithConflictsKnownDependenciesLB.tex <==
\section{Proof of Theorem~\ref{thm:learnAllLBWithConflictsKnownDependenciesLB}}\label{app:learnAllLBWithConflictsKnownDependenciesLB}
\begin{theorem}
	Assume that the repository contains at most $d$ defects and $c$ unknown \textbf{weak} conflicts.
	Any \textbf{non-adaptive} algorithm that solves \learnAll{} must make at least $\parameterizedCFFSize{d+c-1}{2}$ queries.
\end{theorem}
\begin{proof}
	%    Unlike the \maxProblem{} lower bound discussed earlier, for solving \learnAll{} an algorithm must determine whether $p$ is defective, regardless if it is included in a maximal installation.
	%    This allows us to consider the case where $c$ packages $b_1,\ldots,b_c$ directly conflict with $p$ that also have $u$ unknown dependencies on $a_1,\ldots,a_u$. The setting is depicted in Figure~\ref{fig:learnAllLBWithConflicts}.
	Assume by contradiction that the algorithm makes less than $\parameterizedCFFSize{d+c-1}{2}$ queries. 
	This means that there exist a set $S_1=\set{x_1,\ldots,x_{d}}\cup\set{b_1,\ldots,b_{c-1}}$ and  packages $p,q$ such 
	that some tested installation contains $p$ and $q$ but none of $S_1$'s members. 
	We will construct an input scenario for which \learnAll{} cannot be solved
	correctly by this algorithm. Consider the scenario where
	$x_1,\ldots,x_{d}$ are defective packages and $b_1,\ldots,b_{c-1}$ conflict
	with $p$.
	This implies that no installation that contains $p$ \textbf{and} $q$ is tested. Thus, the algorithm cannot determine whether $p$ conflicts with $q$ or not. The setting is depicted in Figure~\ref{fig:learnAllLBWithConflictsKnownDependenciesLBV2}.
		Observe that the number of weak conflicts is at most $c$ as required and there are $d$ defects.
	Thus, the algorithm fails to solve \learnAll{}.
	\begin{figure}[]
		\centering
		\includegraphics[width =
		0.6\columnwidth]{figs/learnAllLBWithConflictsKnownDependenciesLBV2.png}
		
		\caption{If the algorithm makes less than $\parameterizedCFFSize{d+c-1}{2}$
		queries, then there no installation that contains both p and q is tested, thus
		the algorithm can not determine if they are in conflict.
	 }
		\label{fig:learnAllLBWithConflictsKnownDependenciesLBV2}
	\end{figure}
\end{proof}


==> learnAllLBWithConflictsUB.tex <==
\section{Proof of Theorem~\ref{thm:learnAllLBWithConflictsUB}}\label{app:learnAllLBWithConflictsUB}
\begin{theorem*}
	Assume that the repository contains at most $d$ defects, $u$ unknown dependencies and $c$ conflicts.
	There exists a \textbf{non-adaptive} algorithm that solves \learnAll{} using
	\newline $\sum_{i=0}^{u}\parameterizedCFFSize{d+c+(u-i)+1}{i+2}$ queries.
\end{theorem*}
\begin{proof}
	Intuitively, our construction so far was wasteful in the sense that when a test needed to include $p$, we added all its prerequisites to $S_2$ and added every other package with an unknown dependency into $S_1$. While there can be at most $u$ prerequisites to $p$, and at most $p$ other packages with a dependency, we have not used the fact that their \textbf{sum} is also bounded by $u$. That is, assume that $p$ has $i\in\set{0,1,\ldots u}$ prerequisites; then we add $x$ packages to $S_2$ and at most $u-i$ packages to $S_1$. We can use this in the following way -- we construct a set of $u+1$ Cover-Free Families $\set{\CFFLetter_i}_{i=0}^u$ such that $\CFFLetter_i$ is a \parameterizedCFF{d+c+(u-i)+1}{i+2}. We then set the tests of the algorithm to be $\mathcal T\triangleq \bigcup_{i=0}^u \CFFLetter_i$. Similar arguments to those of lemmas~\ref{lem:defectIdentificationWithConflicts},~\ref{lem:learningConflictsWithUnknownDependencies}, and~\ref{lem:learningDependencies} show that we still have witnesses for every non-defective package, every non-conflicting pair of packages and every non-dependent pair. The actual $\CFFLetter_i$ that the relevant test belongs to is the number of prerequisites of the package $p$ in the case of defectiveness and dependency-learning, and the total number of prerequisites of either $p$ or $q$ in the case of determining whether the two conflict.
\end{proof}

==> learningADependency.tex <==
\section{Proof of Theorem~\ref{thm:learningADependency}}\label{app:learningADependency}
\begin{theorem*}
	Assume that no defects or conflicts exist.
	Any non-adaptive algorithm that solves  \learnAll{} must make at least $n-1$
	queries. Note that this holds even when the repository may have only \textit{up
	to} 1 unknown dependency.
\end{theorem*}
\begin{proof}
	Denote $P\triangleq\set{a_1,\ldots,a_n}$ and consider the directed path graph 
	given by $K\triangleq\{(a_i,a_{i-1})\mid i\in\set{2,\ldots,n}\}$. 
	Assume by contradiction that there exists an algorithm that makes 
	less than $n$ queries. In such case, there exists some
	$i\in\set{1,\ldots,n-1}$, such that the installation $\set{1,\ldots, i}$ was not tested. Next, consider two
	possible scenarios -- $U=\set{(a_i,a_n)}$ and $U=\set{(a_{i+1},a_n)}$. That
	is, there is an undocumented dependency of either $a_i$ or $a_{i+1}$ on $a_n$. The setting is illustrated in Figure~\ref{fig:learningDependencyLB}.
	
	Observe that the \emph{only} way to distinguish between the two cases is to try
	the installation $\set{1,\ldots i}$, as all other installations will result in
	the same outcome for both scenarios. Thus, we conclude that the algorithm must try at least $n-1$ queries.
	\begin{figure}[]
		\centering
		\includegraphics[width = 0.6\columnwidth]{figs/learningDependencyLB.png}
		
		\caption{An algorithm that tries to learn a single unknown dependency must differentiate between the case where $a_n$ depends on $a_i$ and the case where it depends on $a_{i+1}$, for every $i\in\set{1,\ldots,n-1}$. This is only possible by trying the installation $\set{1,\ldots i}$.
		}
		\label{fig:learningDependencyLB}
	\end{figure}
\end{proof}



==> learningConflictsWithUnknownDependencies.tex <==
\section{Proof of Lemma~\ref{lem:learningConflictsWithUnknownDependencies}}\label{app:learningConflictsWithUnknownDependencies}
\begin{lemma*}
	Packages $p,q$ weakly conflict iff $S(p)\cap S(q)=\emptyset$.
\end{lemma*}
\begin{proof}
	Similarly to Lemma~\ref{lem:learnConflictsForKnownDependencies}, a pair of conflicting packages $p,q$ cannot be included in a successful test. Here, we show that if no successful installation was tried by the algorithm, then such does not exist and the two packages conflict.
	%Notice that if $p,q$ weakly conflict then no test that contains both can pass and $S(p)\cap S(q)=\emptyset$. 
	In the remainder of the proof, we assume that the two do not conflict and show that the algorithm tries a successful installation that contains both. 
	We define $S_2\triangleq\set{p,q}\cup\set{p'\mid\mbox{$p$ or $q$ has an \textbf{unknown} weak dependency on $p'$}}$ to include $p,q$, and any of their unknown weak prerequisites. We also construct  $S_1\triangleq D\cup X_1\cup X_2\cup X_3$ in a similar manner, where
	\begin{itemize}
		\item $X_1\triangleq \set{x\mid \mbox{($p$ \textbf{and} $q$ do not weakly depend on $x$)}\wedge(\exists p'\in P: (p',x)\in U)}$.
		\item $X_2\triangleq \set{x\mid \exists p':(\set{x,p'}\in C) \wedge(\mbox{$p$ \textbf{or} $q$ weakly depend on $p'$)}}$.
		\item $X_3\triangleq \set{x\mid \exists p':(\set{x,p'}\in C) \wedge\mbox{($p$ \textbf{and} $q$ do not weakly depend on $x$)}\wedge(x\succ p')}$.
	\end{itemize}
	Observe that $|S_1|\le d + c + u<d+c+u+1$ and that $|S_2|\le u+2$. Therefore, there exists a test $v\in\mathcal T$ such that $v\cap S_1=\emptyset$ and $S_2\subseteq v$. The test contains all prerequisites of $p,q$ and satisfies all other constraints. Thus, it passes unless $p,q$ conflict.
\end{proof}

==> learningUnknownDependenciesLemma.tex <==
\section{Proof of Lemma~\ref{lem:learningDependencies}}\label{app:learningDependencies}
\begin{lemma*}
	Package $p$ weakly depends on package $q$ if and only if $S(p)\subseteq S(q)$.
\end{lemma*}
\begin{proof}
	As in the other lemmas, one direction here is straightforward -- if $p$ weakly depends on $q$ then $S(p)\subseteq S(q)$.
	We now construct sets $S_1,S_2$, such that the corresponding test will include $p$, exclude $q$, and pass unless $p$ weakly depends on $q$.
	This is achieved by excluding from the test $q$, and all the packages that weakly depend on it, including $p$ and all its prerequisites, and resolving all unrelated conflicts, dependencies, and defects.
	Formally we set $S_2\triangleq\set{p}\cup\set{p'\mid \mbox{$p$ has a weak dependency on $p'$}}$ to include $p$ and all its prerequisites.
	We define $S_1\triangleq D\cup \set{q}\cup X_1\cup X_2\cup X_3\cup X_4$, where:
	\begin{itemize}
		\item $X_1\triangleq\set{q'\mid \mbox{$q'$ has a weak dependency on $q$}}$
		\item $X_2\triangleq\set{x\mid (\mbox{$p$ does not weakly depend on
		$x$})\wedge(\exists y:(x,y)\in U)}$
		\item $X_3\triangleq \set{x\mid \exists p':(\set{x,p'}\in C) \wedge(\mbox{$p$ weekly depends on $p'$})}$.
		\item $X_4\triangleq \set{x\mid \exists p':(\set{x,p'}\in C) \wedge\mbox{($p$ does not
		 weakly depend on $x$)}\wedge(x\succ p')}$.
	\end{itemize}
	In other words, $X_1$ excludes from the test all packages that weakly depend on $q$; $X_2$ removes all packages with unknown dependencies that are not a prerequisite to $p$; $X_3$ contains all packages that conflict with a prerequisite of $p$; and $X_4$ is the set of packages, chosen according to $\succ$, that is used to resolve conflicts unrelated to $p$.
	An illustration of the setting is depicted in Figure~\ref{fig:learningDependencies}.
	\begin{figure}[]
	\centering
	\includegraphics[width = 0.7\columnwidth]{figs/learningDependencies.png}
	
	\caption{An example of a $S_1,S_2$ whose corresponding test 
		contains $p$ and passes. 
		$S_2$ contains $p$ and its prerequisites, while $S_1$ contains all packages
		that weakly conflict with $p$, $q$ and all those affecting q, and a
		package from each conflict, along with all those that weakly depend on it. 
	}
	\label{fig:learningDependencies}
	\end{figure}	
	Observe that since $|X_1|+|X_2|\le u$, $|X_3|+|X_4|\le c$, we have $|S_1|\le d + 1 + u + c$. Finally, since $|S_2|\le u+1<u+2$ we have that there exists a witness test that addresses all other constraints and passes unless $p$ weakly depends on $q$.
\end{proof}




==> lowerBounds.tex <==
\section{Lower Bounds}
In this section, we provide query lower bounds for the papers studied in this paper. We denote that bounds derived for adaptive algorithms also apply for non-adaptive ones, but not vice versa.
Specifically, we propose an adaptive $\Omega(\bar r\logp{n/\bar r})$ bound when all dependencies are known, matching the query complexity of Algorithm~\ref{alg:basic}. We then show an adaptive $\parameterizedCFFSize{arg1}{arg2}$ lower bound for the general \maxProblem{} problem. This roughly matches the $\parameterizedCFFSize{arg1}{arg2}$ query complexity of Algorithm~\ref{alg:MainMax}. Finally, we show that for a \emph{non-adaptive} bound for a specific family of problem instances while achieving better adaptive query complexity in Algorithm~\ref{alg:adaptive}.

In the following theorem, we assume that we have a bound $r$ on the number of 
\emph{root defects}, no conflicts or unknown dependencies exist, and the overall number of 
defects is not bounded. As the problem forces us to detect all defects, and since the 
problem reduces to group testing for $K=\emptyset$, the following directly follows 
from the group testing lower bound of~\cite{chan}.
\begin{theorem}
	For $\bar{c}=\bar{u}=0$ and $\bar{d}=\infty$, any algorithm for \maxProblem{} requires $\Omega(\bar d\logp{n/d})$ queries.
\end{theorem}

%We now show that when unlike the case of $\bar u=0$ discussed in Theorem~\ref{thm:basicLB} and Algorithm~\ref{alg:basicWithConflicts}, it is not possible to count root defects instead of defects and get a sub linear query complexity in the repository size.


\textbf{Covered in Theorem 4}
Next, we discuss an upper bound for the more general problem where both conflicts and unknown dependencies may be present. Conceptually, we derive the bound for an instance where $K=\emptyset$. Then we claim that each algorithm must use a $\CFF$ to learn the repository as otherwise, it will miss at least one package. The unknown dependencies and conflicts are illustrated in Figure~\ref{fig:maxLB}.
\begin{figure}[t!]
	\centering
	\includegraphics[width = 0.6\columnwidth]{figs/maxLowerBound.png}
	
	\caption{If there exist $S_1,S_2$ such that the algorithm does not have test an installation $I$ for which $S_1\cap I=\emptyset$ and $S_2\subseteq I$ then it can not identify whether $p$ is defective. That is, we consider the case where $x_1,\ldots,x_{d-1}$ are defective, $\set{b_i,a_i}\in C$ for all $i\in\set{1,2,\ldots, c}$, that $(a_j,a_{j-1})\in U$ for all $j\in\set{2,3,\ldots \bar u}$ and that $(a_1,p)\in U$. Thus, in order to identify whether $p$ is defective the algorithm must install $p$ and all $a$'s, and avoid all $x$'s and $b$'s.
	}
	\label{fig:maxLB}
\end{figure}
\begin{theorem}\label{thm:maxLB}
	For any $\bar c, \bar u, \bar d\in\mathbb N$ such that $\bar c\le \bar u$, any algorithm for \maxProblem{} must make at least $\parameterizedCFFSize{\bar c+\bar d-1}{\bar u+1}$ queries.
\end{theorem}
\begin{proof}
	Consider $K=\emptyset$ and $\bar c, \bar u, \bar d\in\mathbb N$ such that $\bar c\le \bar u$. If the algorithm tries less than $\parameterizedCFFSize{\bar c+\bar d-1}{\bar u+1}$ installations then there exist disjoint package sets $S_1,S_2$ of sizes $\bar c+\bar d-1$ and $\bar u+1$ such that no installation included all of $S_2$ and none of the packages in $S_1$. We show that in this case it cannot possibly find the maximal installation for all possible settings. 
	We denote $S_1\triangleq\set{x_1,\ldots x_{d-1}}, \set{b_1,\ldots,b_c}$ and $S_2\triangleq\set{a_1,\ldots a_u}\cup \set{p}$. The set of (unknown) dependencies is $U\triangleq\set{(a_{i+1},a_{i})\mid i\in\set{1,\ldots,u}}\cup \set{(a_1,p)}$, the set of defects includes $\set{x_1,\ldots x_{d-1}}$ and the conflicts are $C\triangleq\set{\set{b_i,a_i}\mid i\in\set{1,\ldots,\bar c}}$.
	Note that thus far $|S_1|=\bar c+\bar d-1,|S_2|=\bar u+1, |U|=\bar u, |C|=\bar c, |D|=\bar d-1$. We now claim that the algorithm cannot possibly distinguish between the case where $p$ is a defect and the case where it is not. Notice that in order for $p$ to be a part of a successful installation, it must contain $S_2$ and none of the packages in $S_1$. Thus, all installations attempted by the algorithm were either unsuccessful or did not contain $p$. Since the same test results would be obtained regardless of whether $p$ is defective, we conclude that the algorithm cannot determine the maximal installation as it must contain $S_2$ if $p$ is working properly.
\end{proof}

Next, we show that for the \learnAll{} problem the bound holds also for $\bar c > \bar u$.
\begin{theorem}
	For any $\bar c, \bar u, \bar d\in\mathbb N$, any algorithm for \learnAll{} must make at least $\parameterizedCFFSize{\bar c+\bar d-1}{\bar u+1}$ queries.
\end{theorem}
\begin{proof}
	In the proof of Theorem~\ref{thm:maxLB} we required $\bar c\le \bar u$ in order for the maximal installation to include $p$ if and only if it is not defective. When the algorithm is required to learn all defective modules, we no longer need $S_2$ to have a cardinality larger than $\bar c$. Thus, we can add as many packages as needed that conflict with $p$ and still require the algorithm to assess whether $p$ is defective.
	Thus, we consider the following scenario:
	$K=\emptyset, S_1\triangleq\set{x_1,\ldots x_{d-1}}\cup\set{b_1,\ldots,b_c}, S_2\triangleq\set{a_1,\ldots,a_{\bar u}}\cup\set{p}, U\triangleq\set{(a_{i+1},a_{i})\mid i\in\set{1,\ldots,u}}\cup \set{(a_1,p)}, C\triangleq\set{\set{b_i,p}\mid i\in\set{1,\ldots,\bar c}}$ and a set of defects that include $\set{x_1,\ldots x_{d-1}}$. The setting is illustrated in Figure~\ref{fig:fullLB}. As before, the algorithm needs to determine whether $p$ is defective but cannot do that as no successful installation that includes $p$ was tried. 
\end{proof}

\begin{figure}[]
	\includegraphics[width = 0.8\columnwidth]{figs/fullLowerBound.png}
	
	\caption{If there exist $S_1,S_2$ such that the algorithm does not have test an installation $I$ for which $S_1\cap I=\emptyset$ and $S_2\subseteq I$ then it can not identify whether $p$ is defective. That is, we consider the case where $x_1,\ldots,x_{d-1}$ are defective, $\set{b_i,a_i}\in C$ for all $i\in\set{1,2,\ldots, c}$, that $(a_j,a_{j-1})\in U$ for all $j\in\set{2,3,\ldots \bar u}$ and that $(a_1,p)\in U$. Thus, in order to identify whether $p$ is defective the algorithm must install $p$ and all $a$'s, and avoid all $x$'s and $b$'s.
	}
	\label{fig:fullLB}
\end{figure}


==> maxLowerBoundWithConflicts.tex <==
\section{Proof of Theorem~\ref{thm:maxLowerBoundWithConflicts}}\label{app:maxLowerBoundWithConflicts}
\begin{theorem*}
	Assume that the repository contains at most $d$ defects, $u$ unknown 
	dependencies, and $c$ unknown \textbf{weak} conflicts.
	For the case that $c\le 2u$, any \textbf{non-adaptive} algorithm that solves
	\maxProblem{} must use $\parameterizedCFFSize{d+\ceil{c/2}-1}{u+1}$ queries.
\end{theorem*}
\begin{proof}
	The setting for the proof is similar to that of
	Theorem~\ref{thm:unknownDependenciesLB} except that there are $\ceil{c/2}-1$
	packages, each conflicting with one of $a_1,\ldots,
	a_{\ceil{c/2}-1}$, therefore they all indirectly conflict with $p$. Another
	package directly conflicts with $p$.
	Formally, if we assume that the algorithm tests less than $\parameterizedCFFSize{d+\ceil{c/2}-1}{u+1}$ installations, 
	there exists a pair of package sets $S_1\triangleq\set{b_1,\ldots,b_{\ceil{c/2}}}\cup\set{x_1,\ldots,x_{d-1}}$ and 
	$S_2\triangleq\set{a_1,\ldots,a_u}\cup\set{p}$ such that no test contains all of $S_2$ but none of the packages in $S_1$. 
	In this case, we prove that the algorithm cannot determine whether $p$ is defective in the following scenario.
	Consider the dependencies $(p,a_1),(p,a_2),\ldots,(p,a_u)$, defects
	$x_1,\ldots,x_{d-1}$ and conflicts $\set{b_1,a_1}, \ldots,\set{b_{\ceil{c/2}-1},a_{\ceil{c/2}-1}},\allowbreak\set{b_{\ceil{c/2}},p}$. 
	The setting is illustrated in Figure~\ref{fig:maxLowerBoundWithConflicts}.
	
	\begin{figure}[]
		\centering
		\includegraphics[width = 0.6\columnwidth]{figs/maxLowerBoundWithConflicts.png}
		
		\caption{If the algorithm makes less than 
		$\parameterizedCFFSize{d+\ceil{c/2}-1}{u+1}$
		queries, it can not determine if $p$ is defective.
		}
		\label{fig:maxLowerBoundWithConflicts}
	\end{figure}
	
	Notice that the number of dependencies is $u$ and that the number of 
	weak conflicts is $c$ (as $\set{b_i,a_i}$ and $\set{b_i,p}$ are 
	weak conflicts for $i\in\set{1,\ldots,\ceil{c/2}-1}$). As in Theorem~\ref{thm:unknownDependenciesLB}, the algorithm 
	has no way to distinguish between the case where $p$ is defective and the case that it is not, 
	as no test that contains $p$ has passed. Finally, notice that the maximal 
	installation contains $a_1,\ldots, a_u$ and potentially $p$, and thus the algorithm fails to solve the problem.
\end{proof}



==> nonAdaptiveAlg.tex <==
\subsection{Non-Adaptive Algorithms}
In this section, we propose a non-adaptive algorithm for \learnAll{}. Intuitively, construct a cover free family, factor in the known dependencies, and get a  set of tests that will later allow us to infer the graph properties. 
In this section, we interchangeably refer to $n$-sized binary vectors as subsets of $P$. Fixing a canonical enumeration of $P$, we say that the $i^{\mathit{th}}$ package is in a vector $v\in\set{0,1}^n$ if its $i^{\mathit{th}}$ bit is set.
Formally, we construct a $\parameterizedCFF{\bar d + \bar c}{\bar u + 1}$ $\CFFLetter$ and define the test set as 
$\mathcal T \triangleq \set{c(v)\mid v\in \mathcal F}$, 
where $c:\set{0,1}^n\to\set{0,1}^n$ is defined as $$c(v)\triangleq\set{p\in P\mid \exists p'\in P, (\mbox{$p$ is reachable from $p'$ in $G_K$})\wedge (v(p')=1)}.$$ 
That is, given a vector $v\in\set{0,1}^n$ we create a test that contains all packages whose bit is set together with those that are a perquisite to a set-bit package. For example, if $P=\set{1,2,3,4}, K=\set{(1,2),(2,3)}$ and $v=\langle0,1,0,0\rangle$ then we test the installation $\set{1,2}$. 
Notice that we can compute the transitive closure of $G_k$ once in 
$O(n^2)$ time and use it to compute $c(v)$ in linear time for every vector 
$v\in\set{0,1}^n$. 

After testing all installations $t\in \mathcal T$, we receive a feedback $f(t)$ of whether $t$ succeeded. We now prove that given $\set{f(t)}_{t\in\mathcal T}$ we can infer all graph properties.
First, for each package $p$ we define its set of successful installations.

\begin{definition}
Given $p\in P$, let $T(p)\triangleq \set{t\in\mathcal T\mid p\in t}$ be the set of tests that installed $p$ and $S(p)=\set{t\in T(p)\mid f(t)=1}$ be the installations that were successful.
\end{definition}
We start by proving that a package is defective only if it was not successfully installed in any of the tests.


\textbf{Covered partially in Theorem 6}
\begin{theorem}\label{thm:defectiveness}
A package $p\in P$ is defective if and only if $S(p)=\emptyset$.
\end{theorem}
\begin{proof}
Recall that a package is defective if there exists no successful installation that contains it. Hence, $p\in D$ immediately implies that $S(p)=\emptyset$. Our goal here is to show the converse -- that $S(p)=\emptyset$ implies that $p$ cannot be a part of any successful installation, including the ones that were not tested by the algorithm.
%Thus, we need to show that if $S(p)=\emptyset$ then no test $t\subseteq P$ that contains $p$ could possibly pass.
%We assume that such $t$ exists and show that it implies $S(p)\neq\emptyset$.

We now disjoint construct sets $S_1,S_2\subseteq P$ of sizes $\bar d + \bar c$ and $\bar u + 1$. From $\CFFLetter$'s properties we are guaranteed that there exists a vector $v\in\CFFLetter$ such that $S_1\cap v=\emptyset$ and $S_2\subseteq v$. We then show that the test $c(v)\in\mathcal T$ passes unless $p$ is defective. We denote by $X(p)\subseteq P$ the set of perquisites of $p$, including both the known and unknown dependencies. That is, $X(p)$ is the set of packages that $p$ is reachable from in $(P,K\cup U)$. Simply put, $X(p)$ is the package set that must be present in any test in $S(p)$.
Notice that by definition, if a package $p'\in X(p)$ is defective then so is $p$. Thus, our test $c(v)$ must contain all packages in $X(p)$. Additionally, if $\set{p',p''}\in C$ for $p',p''\in X(p)$ then $p$ cannot be successfully installed and is considered defective.
Next, any package that conflict with packages of $X(p)$ must be excluded from $c(v)$. For this, we set $S_1\triangleq \set{p'\mid p'\in D}\cup \set{p'\mid \set{p',p''}\in C\wedge p''\in X(p)}\cup \widetilde{C}$. Here, $\widetilde{C}\subseteq P$ is an arbitrary subset of packages that conflict with other packages outside of $X(p)$. That is, for every conflict $\set{p',p''}\in C$ for which $\set{p',p''}\cap X(p)=\emptyset$ we arbitrarily add one of $p',p''$. Next, we define $S_2\triangleq\set{p}\cup\set{p'\in P\mid \exists p''\in X(p), (p',p'')\in U}$. In other words, we add every package $p'$ that has a package $p''\in X(p)$ that depend on it but the dependence was not reported in $K$. Notice that $|S_1|\le \bar c + \bar d$ -- we added all $|D|\le\bar d$ defects and at most a single package from each of the $|C|\le \bar c$ conflicts. Similarly, the size of $S_2$ is at most $\bar u + 1$ as it contains $p$ and perhaps the source of every unknown dependency $(p',p'')\in U$ for some $p''\in X(p)$.

Next, observe that if $p$ is not defective then $c(v)$ must pass. By adding to $S_2\subseteq v$ the package $p$ and all other modules that $X(p)$ depends on, we are guaranteed that $X(p)\subseteq c(v)$. Additionally, we excluded from $v$ (and thus, $c(v)$) all defects as they are in $S_1$. Recall that if the one of the packages in $X(p)$ is defective than so is $p$ and thus $D\cap S_2$ is guaranteed to be empty.
Also, we removed all packages that conflict with a package in $X(p)$ and arbitrarily satisfied the remaining conflicts by choosing one of each pair of conflicting packages.
Since $\CFFLetter$ is sure to include a vector $v$ that satisfies  $S_1\cap v=\emptyset$ and $S_2\subseteq v$, we can asses the defectiveness of $p$ although $D,C$ and $U$ are not known in advance.
Thus, we established that if $p$ is not defective then $c(v)$ must pass.

%Let $S_2\triangleq\set{p}\cup\set{(p'',p')\in U\mid p'\in c(p)}$ be the set of packages that must be installed for $p$ to pass. $S_2$ contains $p$ and all packages that are \emph{unknown} prerequisite to a package in $c(p)$. That is, if a package $p''$ is a perquisite to a known perquisite $p'$ of $p$, then $p''$ is included in $S_2$. 
\end{proof}
\begin{theorem}
A non-defective package $p$ depends on another package $p'$ if and only if $S(p)\subseteq S(p')$.
\end{theorem}
\begin{proof}
As in Theorem~\ref{thm:defectiveness}, one direction here is immediate. Namely, if $p$ depends on $p'$ then no test that contains $p$ but not $p'$ would pass and thus $S(p)\subseteq S(p')$. Our goal is to show that if $S(p)\subseteq S(p')$ then $(p',p)\in U$.
Assume by contradiction that $(p',p)\notin U$; by definition, this means that there exists a successful test $t\subseteq P$

\end{proof}
\begin{theorem}
Two packages $p,p'\in P$ conflict if and only if $S(p)\cap S(p')=\emptyset$.
\end{theorem}
We conclude that given $\set{f(t)}_{t\in\mathcal T}$ one can compute the underlying graph in $O(n^2\parameterizedCFFSize{arg1}{arg2})$ time and with no further queries.

==> notationsTable2.tex <==
\begin{table}[h]
	\centering
	

	
	\begin{tabular}{|c|l|}
		
		\hline
		Symbol & Meaning \tabularnewline
		\hline
		$\mathbb{S}$ & Stream \tabularnewline
		\hline
		$N$ & Current number of packets (in all flows)  \tabularnewline
		\hline
		$H$ & Size of Hierarchy  \tabularnewline
		\hline
		$V$ & Performance parameter, $V\ge H$  \tabularnewline
		\hline
		$S^i_x$ & Variable for the i'th appearance of a prefix $x$. 
		\tabularnewline
		\hline
		$S_{x}$ & Sampled prefixes with id $x$. 
		\tabularnewline
		\hline
		$S$ &  Sampled prefixes from all ids. 
		\tabularnewline
		
		\hline
		$\mathcal U$ & Domain of fully specified items. \tabularnewline
		\hline
		$\epsilon,\epsilon_s,\epsilon_a $ & Overall, sample, algorithm's error guarantee.  \tabularnewline
		\hline
		$\delta,\delta_s , \delta_a$ &   Overall, sample, algorithm confidence. \tabularnewline
		\hline
		$\theta$ & Threshold parameter.    \tabularnewline
		\hline

		$C_{q|P}$ & Conditioned frequency of $q$ with respect to  $P$ \tabularnewline
		\hline
		$G(q|P)$ & Subset of $P$ with the closest prefixes to q.  \tabularnewline
		\hline
		$f_q$ & Frequency of prefix q \tabularnewline
		\hline
		$\widehat{f^{+}_q},\widehat{f^{-}_q}$ & Upper,lower bound for $f_q$  \tabularnewline
		\hline
	\end{tabular}
	\caption{List of Symbols}
	\label{tbl:notations}
	
\end{table}

==> pseudoCode3.tex <==
\section{Pseudocode
for
\learnAll{} with defects and conflicts, when all dependencies are
known}\label{pseudoCode3} \begin{algorithm}[H]
	%    \footnotesize
	\scriptsize
	\begin{algorithmic}[1]
		%\Statex Initialization: $S\gets \emptyset$
		\Function{LearnAll}{$P,K,c,d$} \Comment{At most $c$ weak conflicts and $d$
		defects}
		%\State $S\gets \emptyset$ \Comment{The set of identified non-defect packages}
		\State $D \gets \emptyset$ \Comment{The set of identified defects}
		\State $C \gets \emptyset$ \Comment{The set of identified weak conflicts}
		\State $\CFFLetter \gets CFF(n,d+c,2)$ \Comment{CFF construction}
		\State $\mathcal T \gets \set{c(v)\mid v\in \CFFLetter}$ \Comment{Test vectors
		generated based on all known dependencies}
		\For {$p \in P$ }
			\State $S(p) \gets \emptyset$ \Comment{Successful installations that
			included $p$}
		\EndFor
		\For {$t \in \mathcal T$}
		\State $f(t) \gets Feedback(t)$ \Comment{Get feedback from oracle}
		\If {$f(t)$ = 1} \Comment{Successful installation}
		\For {$p$ tested as part of $t$}
			\State $S(p) \gets S(p) \cup t$
		\EndFor        
		\EndIf
		\EndFor
		
		\For {$p \in P$ }
			\If {$S(p) = \emptyset$} \Comment{No successful installation exists for $p$}
			\State $D \gets D \cup p$
			\EndIf
			\For {$q \in P, q \neq p$}
			\If {$S(p) \cap S(q) = \emptyset$} \Comment{No successful installation exists
			for $p$ and $q$ together} 
			\State $C \gets C \cup \{p,q\}$
			\EndIf
			\EndFor
		\EndFor
		
	
		
		\State\Return $D,C$
		\EndFunction
		
	\end{algorithmic}
	\normalsize
	\caption{\learnAll{} with defects and conflicts, all dependencies are known}
	\label{alg:conflicts_w_unknowns}
\end{algorithm}

==> table_ex.tex <==

 \begin{table*}[t]
	 \footnotesize
 	\addtolength{\tabcolsep}{-0pt} \addtolength{\parskip}{-0.1mm} \center{
 		\begin{tabular}{|c|c|c|c|c|c|}
 			\hline
 			\textbf{Src/Dest } & \textbf{{*}} & \textbf{d1.{*}} & \textbf{d1.d2.{*}} & \textbf{d1.d2.d3.{*}} & \textbf{d1.d2.d3.d4}\tabularnewline
 			\hline
 			\hline
 			\textbf{{*}} & ({*},{*}) & ({*},d1.{*}) & ({*},d1.d2.{*}) & ({*},d1.d2.d3.{*}) & ({*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.{*}} & (s1.{*},{*}) & (s1.{*},d1.{*}) & (s1.{*},d1.d2.{*}) & (s1.{*},d1.d2.d3.{*}) & (s1.{*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.s2.{*}} & (s1.s2.{*},{*}) & (s1.s2.{*},d1.{*}) & (s1.s2.{*},d1.d2.{*}) & (s1.s2.{*},d1.d2.d3.{*}) & (s1.s2.{*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.s2.s3.{*}} & (s1.s2.s3.{*},{*}) & (s1.s2.s3.{*},d1.{*}) & (s1.s2.s3.{*},d1.d2.{*}) & (s1.s2.s3.{*},d1.d2.d3.{*}) & (s1.s2.s3.{*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.s2.s3.s4} & (s1.s2.s3.s4,{*}) & (s1.s2.s3.s4,d1.{*}) & (s1.s2.s3.s4,d1.d2.{*}) & (s1.s2.s3.s4,d1.d2.d3.{*}) & (s1.s2.s3.s4,d1.d2.d3.d4)\tabularnewline
 			\hline
 		\end{tabular}
 		
 		{{\caption{An example of the lattice induced by a two dimensional source/destination byte hierarchy. The top left corner (*,*) is fully general while the bottom right (s1.s2,s3.s4,d1.d2.d3.d4) is fully specified. The parents of each node are directly above it and directly to the left.}
 				\label{tbl:example}
 			}}}
 		\end{table*}
\normalsize

%\begin{figure}[t]
	
%	\center{
%		\includegraphics[width = \columnwidth]{example.png}
%		\caption{\label{fig:example}An illustration of the lattice induced by byte granularity two dimensional hierarchy. Source ip bytes are denoted a1.a2.a3.a4, while destination bytes are denoted b1.b2.b3.b4. The lattice represents all supported queries for this granularity.
%		}}	
%	\end{figure}


==> upperBounds.tex <==
\section{Upper Bounds}
\subsection{Known Dependencies and No Conflicts}

\subsection{Unknown Dependencies Without Conflicts}
In this section, we consider the case where we might have unknown dependencies and defects, but no conflicts exist.
\input{nonAdaptiveAlg}
\subsection{Addressing Conflicts}
In the previous section we assumed that no conflicts exist ($\bar c = 0$). However, this assumption might not be realistic and new packages could conflict with each other or existing modules. Thus, we here address the case where $\bar{u}=0, \bar{c}>0$ and $\bar{d}=\infty$. Thus, we have to handle up to $\bar c$ conflicts and $r$ root defects while knowing all dependencies. 
%For this we propose an algorithm that iteratively finds a defect or a conflict in $O(\log n)$ queries. Thus, the overall query complexity becomes $O((r+c)\log n)$ for \learnAll{}.
%Intuitively, at each step we split the set of suspected packages in half, testing each separately and all combined. 
%The equal partition here, unlike the $2^\alpha$-sized test of the previous algorithm, 

For this we propose a non-adaptive, CFF-based, algorithm. Let $\mathcal F$ be a \parameterizedCFF{2}{r+c} CFF. As mention in Section~\ref{sec:CFFs}, we can efficiently construct $\mathcal F$ of size $\parameterizedCFFSize{2}{r+c}=(r+c)^{3+o(1)}\log n$ in linear time. Given $\mathcal F$ we design a test suite that depend on $K$. Then, given the feedback for the tests we can extract all conflicts. 
Finding the optimal \maxProblem{} solution \emph{given the conflicts} is a NP-hard problem as essentially we are looking for a Maximal Independent set under the conflict edges. Nevertheless, if $c$ is small we can solve this problem in practice. First, there exists a simple $O(2^c\cdot c\cdot |P|)$ algorithm that goes over all $2^c$ possibilities to resolve the conflicts and then remove all packages that depend on the removed modules. Alternatively, it was suggested that conflicts in software repository often admit a structure which allows this problem to be efficiently 
optimized using a SAT solver~\cite{Mancinelli2006}.


\begin{algorithm}[H]
	%	\footnotesize
	\scriptsize
	\begin{algorithmic}[1]
		%\Statex Initialization: $S\gets \emptyset$
%		\Function{Test}{$P,K,\bar r$}\Comment{Find at most $r$ root defects in $P$}
		\Function{Learn}{$P,K$}\Comment{Find at most $r$ root defects in $P$}
		\State $S\gets \emptyset$ \Comment{The set of identified non-defect packages}
		\State $R \gets \emptyset$ \Comment{The set of identified root defects}
		\State $\mathcal C\gets \emptyset$ \Comment{The set of identified conflicts}
		%		        \State $n \gets |P|$ \Comment{The remaining number of packages to test}
%		\State $\mathfrak r \gets \bar r$ \Comment{A bound on the number of unidentified root defects}
		\State $X \gets P$ \Comment{The test of untested packages}
		\State $L \gets \text{Topolocial Sort}(P,K)$
		%		        \State $\reachabilityMap \gets \text{Reachable vertices map}(P,K)$.\Comment{\textbf{TODO: consider removing}}
		%		        \While {$n \le 2d-2$}
		\While {$\mbox{test}(X)$ fails}
		\State $T \gets \mbox{An $|X|/2$-sized subset of $X$ with minimal $L$ indices}$
		\If{$\mbox{test}(T\cup S)$ fails} \Comment{Test $T\cup S$}
		\State $p \gets \mbox{\sc {FindSingleDefect}}(T)$ \Comment{Find a root defect using $\alpha$ tests}
		\State $R\gets R\cup \set{p}$
		\State $X\gets  X \setminus\set{p'\in P\mid p'\mbox{ is reachable from $p$ in }(P,K)}$ \Comment{Remove all packages that depend on $p$}
		\State $\mathfrak r\gets \mathfrak r-1$
		\Else\Comment{If the test succeeded}
		\State $S \gets S \cup T$
		%		        		\State $X\gets  X\cup S$      		
		\EndIf
		%		        		\State $n\gets|X|$		  		        	
		\State $X\gets  X \setminus S$ \Comment{Remove newly discovered working packages from $X$}
		\EndWhile
		\For {$p\in X$, in an increasing order of $L$}% \Comment{In an increasing order of $L$}
		\If {$(\set{p}\cup S)$ fails} \Comment{Test $\set{p}\cup S$}
		\State $R\gets R\cup \set{p}$
		\State $X\gets  X \setminus\set{p'\in P\mid p'\mbox{ is reachable from $p$ in }(P,K)}$\Comment{Can be computed using BFS}
		%		        		\State $d\gets d-1$
		\Else
		\State $S\gets S \cup \set{p}$
		\EndIf
		\EndFor
		\State\Return $R$
		\EndFunction
		
		\Function{FindSingleDefect}{$T$}
		\State $A \gets T$ \Comment{The set of suspicious packages}
		\While {$|A|>1$}
		\State $B \gets \mbox{An $|A|/2$-sized subset of $A$ with minimal $L$ indices}$        	
		\If{$(B\cup S)$ fails}\Comment{Test $B\cup S$}
		\State $A\gets B$
		\Else\Comment{If the test succeeded}
		\State $S \gets S \cup B$
		\State $A \gets A\setminus B$	        	
		\EndIf	
		\EndWhile
		\State\Return $p\in A$ \Comment{The remaining package is guaranteed to be a root defect.}
		\EndFunction        
		%		\State
	\end{algorithmic}
\normalsize
\caption{Identifying root defects given all dependencies in the presence of conflicts}
\label{alg:basicWithConflicts}
\end{algorithm}

\subsection{Adaptive Algorithms}
\begin{algorithm}[h]
	%\footnotesize
	\begin{algorithmic}[1]
		%\Statex Initialization: $\forall d\in[L]: HH[d] =$ HH\_Alg $(\epsilon_a^{-1})$
		%        \Function{Update}{ $x$}
		%        \State $d = randomInt(0,V)$
		%        \If {$d<H$}
		%        \State Prefix $p = x\&HH[d].mask$ \Comment{Bitwise AND}
		%        \State $HH[d].INCREMENT(p)$
		%        \EndIf
		%        \EndFunction
		%
		%        \Function{Output}{$\theta$}
		%        \State $P = \phi$
		%        \For{Level $l = |H|$ down to $0$. }
		%        \For{ each $p$ in level $l$}
		%        \State \label{line:cp}$\widehat{C_{p|P}} = \widehat{f_p}^{+} + calcPred(p,P) $
		%        \State \label{line:accSample}$\widehat{C_{p|P}} = \widehat{C_{p|P}}+ 2{{Z_{1 - {\delta}}}\sqrt {NV} }$
		%        \If {$\widehat{C_{p|P}}\ge \theta N$}
		%        \State $ P = P \cup \{p\}$ \Comment{$p$ is an HHH candidate}
		%        \State $print\geft(p, \widehat{f_p}^{-}, \widehat{f_p}^{+}\right)$
		%        \EndIf
		%        \EndFor
		%        \EndFor
		%        \State\Return $P$
		%        \EndFunction
		\State
	\end{algorithmic}
	\normalsize
	\caption{}
	\label{alg:Skipper}
\end{algorithm}

